Quartz Clouds in the Dayside Atmosphere of the Quintessential Hot Jupiter HD 189733 b

Recent mid-infrared observations with JWST/MIRI have resulted in the first direct detections of absorption features from silicate clouds in the transmission spectra of two transiting exoplanets, WASP-17 b and WASP-107 b. In this paper, we measure the mid-infrared ($5-12$ $\mu$m) dayside emission spectrum of the benchmark hot Jupiter HD 189733 b with MIRI LRS by combining data from two secondary eclipse observations. We confirm the previous detection of H$_2$O absorption at 6.5 $\mu$m from Spitzer/IRS and additionally detect H$_2$S as well as an absorption feature at 8.7 $\mu$m in both secondary eclipse observations. The excess absorption at 8.7 $\mu$m can be explained by the presence of small ($\sim$0.01 $\mu$m) grains of SiO$_2$[s] in the uppermost layers of HD 189733 b's dayside atmosphere. This is the first direct detection of silicate clouds in HD 189733 b's atmosphere, and the first detection of a distinct absorption feature from silicate clouds on the day side of any hot Jupiter. We find that models including SiO$_2$[s] are preferred by $6-7\sigma$ over clear models and those with other potential cloud species. The high altitude location of these silicate particles is best explained by formation in the hottest regions of HD 189733 b's dayside atmosphere near the substellar point. We additionally find that HD 189733 b's emission spectrum longward of 9 $\mu$m displays residual features not well captured by our current atmospheric models. When combined with other JWST observations of HD 189733 b's transmission and emission spectrum at shorter wavelengths, these observations will provide us with the most detailed picture to date of the atmospheric composition and cloud properties of this benchmark hot Jupiter.

==> scratch <==
We compare our emission spectrum of HD 189733 b to a grid of 1D radiative–convective–thermochemical–equilibrium (RCTE) model grids generated by \texttt{PICASO} for the parameters for HD 189733 b. In Fig.\ref{fig:T_bright} we plot the best fit model to our eclipse spectrum. We detect gas phase absorption features only from H$_2$O. We see no evidence of absorption from any carbon carrying species: CO$_2$,CH$_4$ or CO. Because of this, we are unable to put constrain the C/O or metallicity of HD 189733 b from the MIRI data alone.

We test dozens of different gas phase and condensate species in order to fit the unknown absorption features at $8.7$ $\mu$m and 9.3 $\mu$m. \textbf{list? Waiting on collaborators to check opacities}

SiO$_2$ has a prominent feature at 8.7 microns, however, when we plot the condensation curve for SiO$_2$ against the average dayside temperature profile from forward models of HD 189733 b (Fig.~\ref{fig:T_bright}b), we find a predicted condensation pressure deeper than the photosphere. However, there may be local hotspots on the dayside when the temperature is hot enough that quartz grains may condense in the observable atmosphere. We therefore post process Si$_O$ particles into our forward models using \texttt{Virga} \textbf{(citation)} and perform a grid-trieval varying the sedimentation efficiency, f$_{sed}$, cloud base pressure, width of the particle size distribution, and the number density of particles. 

We find that the data prefer the inclusion of SiO$_2$ grains in the atmosphere at 4$\sigma$ (Bayes factor = 610). In order to reproduce the observed feature, we require a very low sedimentation efficiency, f$_{sed}\approx0.15$. The retrieved base pressure is at 10$^{-4}$ bars, substantially higher in the atmosphere then predicted by the condensation curves. 
